Dronevision: An Experimental 3D Testbed for Flying Light Specks

Today's robotic laboratories for drones are housed in a large room. At times, they are the size of a warehouse. These spaces are typically equipped with permanent devices to localize the drones, e.g., Vicon Infrared cameras. Significant time is invested to fine-tune the localization apparatus to compute and control the position of the drones. One may use these laboratories to develop a 3D multimedia system with miniature sized drones configured with light sources. As an alternative, this brave new idea paper envisions shrinking these room-sized laboratories to the size of a cube or cuboid that sits on a desk and costs less than 10K dollars. The resulting Dronevision (DV) will be the size of a 1990s Television. In addition to light sources, its Flying Light Specks (FLSs) will be network-enabled drones with storage and processing capability to implement decentralized algorithms. The DV will include a localization technique to expedite development of 3D displays. It will act as a haptic interface for a user to interact with and manipulate the 3D virtual illuminations. It will empower an experimenter to design, implement, test, debug, and maintain software and hardware that realize novel algorithms in the comfort of their office without having to reserve a laboratory. In addition to enhancing productivity, it will improve safety of the experimenter by minimizing the likelihood of accidents. This paper introduces the concept of a DV, the research agenda one may pursue using this device, and our plans to realize one.

==> hardware.tex <==
\subsection{Challenges of Small Drones}
\subsubsection{Physical Limits} (Yang Singh)


%While drone swarms forming Flying Light Specks (FLS) can create complex 3D visualizations and haptic feedback, limitations apply to the system that the drone community is facing as well. 



%Battery life limits the duration of a display, which is another constraint that needs to be addressed for DV. Research of drone powering methods has shown the possibility of continuous operation, using laser, drone swapping, or tethered drones \cite{Swieringa, Frédéric, Achtelik, Ouyang}. DV will adopt a drone-swapping approach to enable continuous operation. A limitation of the drone-swapping technique could mean that the formation needs to be reconfigured when drones are low on battery and need to be recharged. 

Additionally, the force exerted by the drones may not be sufficient to provide robust haptic feedback.
The size of the drone is a trade-off between the payload thrust versus the rendering resolution of the FLS. 
Small drones could have more rendering resolution, but would drastically decrease the thrust to handle the haptic of the FLS as the propeller size are small. 


\subsubsection{Coordination and Flight Formation} 

The coordination and flight formation of Flying Light Specks (FLS) to render a sphere faces inherent constraints due to the physical characteristics of drones. A drone's limited turning radius and its ability to manage downwash, the air displaced by the drone's rotors, set a limit on the smallest radius of the sphere that can be rendered. Our pilot study showed that we are able to fly 3 drones following a xy-plane circle path within a radius of 0.5 meters at 1 meter per second. To effectively follow path plans, drones require an understanding of their external state, which includes factors such as downwash and the need for sufficient clearance from the drone in front. This clearance ensures that each drone maintains a safe minimum distance from its neighbor, avoiding potential collisions and mitigating the effects of downwash. Furthermore, the path planning process should ideally be designed with ease of changeability in mind. This would empower users to implement their own path plans with minimal effort, offering a more flexible and customizable FLS experience.





==> infra.tex <==
%\begin{itemize}
   % \item Standards for FLSs. (Shahram)
 %   \item Peripheral devices:  Interoperability with 3D cameras and other devices. (Shahram)
    %\item Audio:  Cause of the noise, Active noise supression/cacnellation, 3D audio, out-of-the box thinking with headsets/earphones (Shahram, Yang)
%\end{itemize}

A DV Hub will support both depth cameras and 3D audio, see Figure~\ref{fig:depthcam}.
This section describes these peripheral devices in turn.

\noindent{\em Depth Cameras.} 
Depthcams are devices that sense the 3D depth of a scene and record it.  
These devices may be categornized into those that use either Time-of-Flight (ToF), Triangulation, or both~\cite{shahram2021}.
For example, Microsoft's Kinect One uses a flash of light to illuminate a scene and thousands of sensors measure the return time from different parts of the scene.  
This pixelated ToF device measures depth of a million points per second.
The D4xx series of Intel RealSense~\cite{realsense2020} depthcams use triangulation technique via stereoscopic imaging.
It uses two cameras to record a scene and compare image patches from one camera with image patches in the other camera to collect depth data.
The basic idea is that those objects that are closer to the camera are displaced more in the horizontal axis.
Cameras such as Intel RealSense D43x and D45x depthcams combine a ToF technique using infrared (IR) light with the triangulation technique to acquire depth data more accurately.
A depthcam may store its recorded data on its local storage.

A DV Hub will have interfaces for users to plug-in a depthcam to stream its captured data for display in real time.  This data may be streamed from the local storage of the depthcam.  The user may copy the data onto the DV Hub's storage for display at a later time. 

Display of streamed depthcam data requires the DV Hub to compute flight paths for FLSs.
Motill~\cite{shahram2022} is an algorithm that processes a sequence of mesh point clouds to compute the flight path for FLSs.
Its complexity is a function of the number of points that constitutes each point cloud. 
It is highly parallelizable and may use multiple cores to compute the FLS flight paths. 
These flight paths may be stored in a bag file~\cite{mmsys2023} for future recall, eliminating the need to re-compute flight paths for a repeated display of point cloud sequence.

\noindent{\em 3D Acoustics.}


==> logc.tex <==
\section{Logging Component}\label{sec:logc}
LogC constructs a log file for each memtable and generates a log record prior to writing to the memtable. 
LogC approximates the size of a log file to be the same as the memtable size.  
A log record is self-contained and is in the form of (log record size, memtable id, key size, key, value size, value, sequence number).  

The log file may be either in memory (availability) or persistent (durability). 
It may be configured to be persistent while its most recent log records are maintained in memory.  
This reduces mean-time-to-recovery of an LTC, enhancing availability while implementing durability.  
An in-memory log file may be replicated to enhance its availability.  
If all in-memory replicas fail, there is data loss. 
Next section describes our implementation of these alternatives. 


==> plan.tex <==
   
    
To realize a prototype of a Dronevision, our research currently focuses on the following main components: Drone localization, control and disturbance balancing, user safety, and continuous charging. 
In regards to drone control and disturbance, we are currently designing a residual PID system that follows the computed path and renders the target force output. We are also investigating in how far can drones be away from each other while having the presence of a cage. We are currently conducting experiments with S500 drone frames fitted with Pixhawk p6x, 920kV motors, and 4 ESCs. As the drone needs to be fitted with a cage to ensure human safety, we are also investigating the performance of the drone system while having a cage/mesh around propellers. 

We are currently using a motion tracking system that provides the position ground truth for the drone's pose and human gesture. Using such Vicon external tracking system, we have set up a drone system to achieve centimeter-level tracking accuracy.

     
Both flights with small drones and balancing with human haptic inputs are required. As of today's propeller technology, using a small drone to generate kinesthetic feedback is hard.
     
     
We have instead used an S500 quadcopter which provides enough additional thrust to render the necessary haptics feedback. The quadcopter could provide x (will conduct experiment tomorrow) grams of thrust, with the drone weighing  

%What is our research agenda to realize a prototype of a Dronevision.

%\begin{itemize}
%    \item How the change in one component impact others?  This is to empower an experimenter to know what can be changed with limited impact on the rest of the system. 
%\end{itemize}

==> software.tex <==
\begin{itemize}
    \item Content rendering tools:  How does a Dronevision render an authored animated sequence? (Shahram)
    \item Decentralized algorithms:  STAG, Failure handling, collision avoidance.  (Hamed, Shuqin and Shahram)
\end{itemize}




==> systems.tex <==
%\begin{itemize}
    %\item Operating system. (Shahram)

    %\item Network.  (Hamed, Shahram)
    %\item Storage:  Data management and sharing. (Shahram)
    %\item State Machine (Shahram, Hamed)
   % \item Failure handling - how to replace failed FLSs?  How to troubleshoot the hardware and software? (Hamed, Shahram)
%\end{itemize}

We will use an off-the-shelf Operating System, OS, for both the DV Hub and an FLS.
The Hub resembles today's servers with adequate resources.
However, an FLS is resource constrained.
It shares similarities with a sensor in a wireless sensor network~\cite{Levis2005,Farooq2011OperatingSF} or a device in an Internet-of-Things, IoT~\cite{}.
It is different because it operates in a well defined indoor environment, the DV display.

The ideal OS for an FLS will have a small memory footprint, be energy efficient, provide real time capabilities, network connectivity, and support heterogeneous devices that may be connected to an FLS (e.g., cameras, sensors to localize an FLS).
An experimenter will use the DV Hub to download and install firmware and device drivers on one or more FLSs and finetune their settings.

%Network:  UDP with packet loss.
FLSs will communicate with one another and the Hub to implement a variety of centralized and decentralized algorithms for charging their battery, localization, collision avoidance, failure handling, haptics, etc.
We will use UDP (or a network protocol similar to UDP) to facilitate this communication.
Features of UDP include its unreliable packet delivery and out of order delivery of transmitted packets to a recipient.
It is the responsibility of an application to use these features effectively. 

We use a finite state machine with an event driven framework to implement FLS functionality using UDP.  
This framework represents an FLS as an abstract machine that can be in exactly one of a finite number of states at any given time.
An event handler processes a queue of events that transitions the state of this abstract machine, an FLS.
It processes events sequentially and atomically, preventing undesirable race conditions caused by inter-leaved execution of two or more events.

%This multi-threaded framework consists of worker threads. 
%A worker thread may read the state of the machine.  To write the state, a thread must generate an event and insert it in the event queue.
%These threads process incoming messages or monitor the clock to generate events. 
%However, only the event handler processes events by reading and transitioning the state of the machine.
%This simplifies the implementation of algorithms.

An FLS may have several independent state machines, event queues, and event handlers that implement mutually exclusive functionalities.
For example, localization, collision avoidance, failure handling, and haptics may be implemented as four different state machines. 
There will be four event queues and four event handlers.
We will use the real time capabilities of the OS to prioritize event handlers. 
For example, the handler that detects and avoids collisions with a user and other FLSs may be given the highest priority~\cite{reynolds87} when compared with other handlers.

Using the Python programming language, we have implemented a scalable emulator with processes where each process represents an FLS.
The processes communicate using UDP.  
Each process implements the aforementioned state machines with an event queue and event handlers.  
At the time of this writing, we have an implementation of a decentralized localization technique, a centralized and decentralized FLS group formation technique, and a decentralized collision avoidance technique.
The emulator scales both vertically and horizontally.  
We have conducted experiments using servers with both a few number of cores (8) and many (72) cores.  We have also conducted experiments with the emulator running on many multi-core servers.  

With the Hub and real-time feeds from a depth camera (see Figure~\ref{fig:depthcam}), we use
Motill~\cite{shahram2022} to processes its sequence of mesh point clouds to compute the flight path for FLSs.
Its complexity is a function of the number of points that constitutes each point cloud. 
Motill is highly parallelizable and may use multiple cores to compute the FLS flight paths. 
These flight paths may be stored in a bag file~\cite{mmsys2023} for future recall, eliminating the need to re-compute flight paths for a repeated display of point cloud sequence.

